Category-level Text-to-Image Retrieval Improved: Bridging the Domain Gap with Diffusion Models and Vision Encoders

This work explores text-to-image retrieval for queries that specify or describe a semantic category. While vision-and-language models (VLMs) like CLIP offer a straightforward open-vocabulary solution, they map text and images to distant regions in the representation space, limiting retrieval performance. To bridge this modality gap, we propose a two-step approach. First, we transform the text query into a visual query using a generative diffusion model. Then, we estimate image-to-image similarity with a vision model. Additionally, we introduce an aggregation network that combines multiple generated images into a single vector representation and fuses similarity scores across both query modalities. Our approach leverages advancements in vision encoders, VLMs, and text-to-image generation models. Extensive evaluations show that it consistently outperforms retrieval methods relying solely on text queries. Source code is available at: https://github.com/faixan-khan/cletir

==> tables/add_exp.tex <==
% \begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrlr}
\rotatebox{90}{Aggregator} & \rotatebox{90}{Backbone} & \rotatebox{90}{Generator }& \rotatebox{90}{ImageNet} & \rotatebox{90}{DTD} & \rotatebox{90}{Stanford Cars}     & \rotatebox{90}{SUN397}   & \rotatebox{90}{Food}     & \rotatebox{90}{FGVC Aircraft} & \rotatebox{90}{Oxford Pets}     & \rotatebox{90}{Caltech101} & \rotatebox{90}{Flowers 102}  & \rotatebox{90}{UCF101}      & \rotatebox{90}{Kinetics-700}    & \rotatebox{90}{RESISC45}      & \rotatebox{90}{CIFAR-10}      & \rotatebox{90}{CIFAR-100}     & \rotatebox{90}{Places-365} & \rotatebox{90}{Average} \\
\midrule
$a_\theta$ & DinoV2~\cite{oquab2023dinov2} & SD~\cite{sd} & 73.8 & 50.1 & 67.1 & 62.4 & \textbf{90.7} & \textbf{29.1} & 91.0 & 93.1 & 79.6 & \textbf{72.5} & 40.8 & \textbf{66.6} & 90.4 & 80.4 & 31.9 & \textbf{68.0} \\


$a_\theta$ & DeiT-III~\cite{deit3} & SD~\cite{sd} & \textbf{80.3} & 47.5 & 64.3 & 60.9 & 88.7 & 28.8 & 91.1 & 92.8 & 78.2 & 70.5 & 39.0 & 66.2 & 91.5 & \textbf{80.7} & 30.9 & 67.4 \\
\midrule
$a_\theta$  & DinoV2~\cite{oquab2023dinov2} & FLUX~\cite{flux} & 71.7 & 48.7 & \textbf{69.7} & 61.5 & 89.0 & 27.9 & \textbf{92.6} & \textbf{93.4} & 75.6 & 71.2 & 40.4 & \textbf{66.6} & \textbf{92.4} & 79.0 & 31.5 & 67.4 \\
$a_\theta$ & DinoV2~\cite{oquab2023dinov2} & SD-Turbo~\cite{add} & 73.7 & \textbf{51.2} & 65.3 & \textbf{63.3} & 90.4 & 28.8 & 92.1 & 93.3 & \textbf{80.3} & 71.7 & \textbf{41.2} & 65.7 & 91.8 & 79.7 & \textbf{32.3} & \textbf{68.0} \\
\midrule
\end{tabular}
}
% \end{table*}

==> tables/corruption.tex <==
% \begin{table*}[]
% \resizebox{\textwidth}{!}
\centering
{
\footnotesize
\begin{tabular}{lrrrrrrrrrrrrrrlr}
& \rotatebox{90}{ImageNet} & \rotatebox{90}{DTD} & \rotatebox{90}{Stanford Cars}     & \rotatebox{90}{SUN397}   & \rotatebox{90}{Food}     & \rotatebox{90}{FGVC Aircraft} & \rotatebox{90}{Oxford Pets}     & \rotatebox{90}{Caltech101} & \rotatebox{90}{Flowers 102}  & \rotatebox{90}{UCF101}      & \rotatebox{90}{Kinetics-700}    & \rotatebox{90}{RESISC45}      & \rotatebox{90}{CIFAR-10}      & \rotatebox{90}{CIFAR-100}     & \rotatebox{90}{Places-365} & \rotatebox{90}{Average} \\
\midrule
text-only(M) & 66.5 & 39.8 & 73.8 & 56.0 & 88.5 & 31.4 & 88.7 & 91.5 & 74.9 & 65.7 & 35.9 & 55.4 & 88.5 & 67.2 & 26.6 & 63.4\\
image-only(M) & 34.9 & 20.9 & 35.7 & 35.1 & 58.6 & 15.7 & 52.0 & 74.3 & 35.1 & 46.3 & 18.6 & 33.4 & 74.8 & 48.9 & 16.7 & 40.1\\
text(M) + image(M) & 54.1 & 32.4 & 54.7 & 50.2 & 81.5 & 22.4 & 75.4 & 87.4 & 62.0 & 61.8 & 30.4 & 53.0 & 88.5 & 64.3 & 23.7 & 56.1\\
text(M) + image(D) & 69.9 & 46.0 & 57.2 & 57.2 & 83.7 & 23.9 & 89.0 & 91.8 & 76.9 & 65.6 & 34.3 & 54.7 & 79.0 & 81.7 & 30.3 & 62.7\\
\rowcolor{blond}
Ours & \textbf{74.2} & \textbf{48.5} & \textbf{74.1} & \textbf{63.2} & \textbf{90.3} & \textbf{33.7} & \textbf{91.5} & \textbf{94.3} & \textbf{79.3} & \textbf{71.9} & \textbf{40.3} & \textbf{59.2} & \textbf{90.2} & \textbf{83.0} & \textbf{32.2} & \textbf{68.4}\\
\midrule


text-only(O) & 63.4 & 38.6 & \textbf{83.1} & 59.8 & 86.8 & 20.9 & 86.2 & 90.9 & 71.0 & 65.7 & 32.7 & 67.1 & 93.3 & 70.0 & 29.6 & 63.9\\
image-only(O) & 41.0 & 31.2 & 52.6 & 45.7 & 66.1 & 13.9 & 58.2 & 79.9 & 50.1 & 50.8 & 21.4 & 51.2 & 82.2 & 53.9 & 22.8 & 48.1\\
text(O)+image(O) & 56.1 & 39.8 & 70.4 & 56.2 & 80.6 & 19.3 & 75.6 & 87.6 & 65.3 & 61.2 & 29.9 & 62.3 & 92.1 & 66.8 & 28.4 & 59.4\\
text(O)+image(D) & 70.3 & 46.3 & 50.7 & 59.5 & 82.9 & 16.3 & 88.2 & 92.7 & 73.8 & 66.7 & 34.6 & 62.8 & 94.5 & 84.9 & 32.3 & 63.8\\
\rowcolor{blond}
Ours & \textbf{70.8} & \textbf{45.0} & 82.2 & \textbf{63.4} & \textbf{89.0} & \textbf{23.0} & \textbf{89.2} & \textbf{93.1} & \textbf{74.9} & \textbf{69.8} & \textbf{36.9} & \textbf{67.8} & \textbf{94.5} & \textbf{80.0} & \textbf{32.7} & \textbf{67.5} \\
\midrule



text-only(E) & 71.1 & 43.9 & \textbf{83.6} & 62.2 & 90.4 & 30.6 & 89.4 & 93.6 & 77.8 & 70.0 & 42.6 & 68.0 & \textbf{97.4} & 86.9 & 29.5 & 69.1\\
image-only(E) & 39.8 & 24.7 & 50.5 & 41.4 & 65.7 & 14.9 & 60.2 & 78.6 & 55.9 & 50.0 & 23.5 & 43.4 & 81.6 & 69.3 & 19.6 & 47.9\\
text(E)+image(E) & 55.9 & 32.5 & 66.9 & 52.7 & 83.1 & 20.9 & 78.1 & 87.4 & 71.1 & 60.5 & 32.9 & 57.7 & 88.8 & 79.8 & 25.7 & 59.6\\
text(E)+image(D) & 69.8 & 44.9 & 45.8 & 57.8 & 81.9 & 17.0 & 87.9 & 91.9 & 73.7 & 65.6 & 34.2 & 58.5 & 91.4 & 85.4 & 31.1 & 62.4\\
\rowcolor{blond}
Ours & \textbf{75.9} & \textbf{51.2} & 82.4 & \textbf{65.0} & \textbf{91.3} & \textbf{31.2} & \textbf{90.7} & \textbf{94.6} & \textbf{79.9} & \textbf{73.1} & \textbf{43.0} & \textbf{68.5} & 95.3 & \textbf{89.8} & \textbf{33.5} & \textbf{71.0}\\
\midrule
\end{tabular}
% \label{tab:baselines}
}
% \end{table*}

==> tables/vague.tex <==
\setlength{\tabcolsep}{4pt}
\small
\centering % used for centering table
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{\msp}ccccccccccccccccc} % 
% \toprule
 Variant & Method & \rotatebox{90}{ImageNet} & \rotatebox{90}{DTD} & \rotatebox{90}{Stanford Cars}     & \rotatebox{90}{SUN397}   & \rotatebox{90}{Food}     & \rotatebox{90}{FGVC Aircraft} & \rotatebox{90}{Oxford Pets}     & \rotatebox{90}{Caltech101} & \rotatebox{90}{Flowers 102}  & \rotatebox{90}{UCF101}      & \rotatebox{90}{Kinetics-700}    & \rotatebox{90}{RESISC45}      & \rotatebox{90}{CIFAR-10}      & \rotatebox{90}{CIFAR-100}     & \rotatebox{90}{Places-365} & \rotatebox{90}{Average} \\

\midrule
\multirow{4}{*}{Description-Only} &
text-only (C) & 34.4 & 23.4 & 8.5 & 38.1 & 67.9 & 12.6 & 21.3  &  76.4 & 35.2 & 48.0 & 18.5 & 42.4 & 73.1 & 42.3 & 16.2 & 37.2 \\
% \rowcolor{blond}
& \cellcolor{blond}Ours (C,D) & \cellcolor{blond}\textbf{42.4} & \cellcolor{blond}\textbf{29.5} & \cellcolor{blond}\textbf{10.1} & \cellcolor{blond}\textbf{45.5} & \cellcolor{blond}\textbf{71.5} & \cellcolor{blond}\textbf{13.6} & \cellcolor{blond}\textbf{32.5} & \cellcolor{blond}\textbf{82.2} & \cellcolor{blond}\textbf{41.5}  & \cellcolor{blond}\textbf{57.2} & \cellcolor{blond}\textbf{24.8} & \cellcolor{blond}\textbf{47.8} & \cellcolor{blond}\textbf{79.0} & \cellcolor{blond}\textbf{55.5} & \cellcolor{blond}\textbf{21.3} & \cellcolor{blond}\textbf{43.6} \\
& text-only (S) & 46.9 & 32.7 & \textbf{12.3} & 42.5 & \textbf{79.8} & 14.2 & 37.1 & 80.0 & 43.5  & 53.4 & 26.8 & 47.5 & 75.3 & 57.4 & 20.3 & 44.6 \\
% \rowcolor{blond}
& \cellcolor{blond}Ours (S,D)& \cellcolor{blond}\textbf{49.9} & \cellcolor{blond}\textbf{35.3} & \cellcolor{blond}12.1 & \cellcolor{blond}\textbf{47.3} & \cellcolor{blond}77.7 & \cellcolor{blond}\textbf{14.9} & \cellcolor{blond}\textbf{44.1} & \cellcolor{blond}\textbf{85.1} & \cellcolor{blond}\textbf{48.3}  & \cellcolor{blond}\textbf{61.4} & \cellcolor{blond}\textbf{30.1} & \cellcolor{blond}\textbf{50.5} & \cellcolor{blond}\textbf{78.9} & \cellcolor{blond}\textbf{63.8} & \cellcolor{blond}\textbf{23.9} & \cellcolor{blond}\textbf{48.2} \\
\bottomrule

\multirow{4}{*}{Description + Class} &
text-only (C) & 65.5 & \textbf{47.0} & 66.2 & 53.5 & 90.4 & \textbf{30.8} & 85.2  & 93.4 & 80.4 & 66.6 & 31.4 & 54.6 & 94.4 & 70.0 & 24.5 & 63.6 \\
% \rowcolor{blond}
& \cellcolor{blond}Ours (C,D) & \cellcolor{blond}\textbf{71.8} & \cellcolor{blond}46.8 & \cellcolor{blond}\textbf{66.8} & \cellcolor{blond}\textbf{58.1} & \cellcolor{blond}\textbf{90.8} & \cellcolor{blond}29.7 & \cellcolor{blond}\textbf{91.2} & \cellcolor{blond}\textbf{95.4} & \cellcolor{blond}\textbf{82.2}  & \cellcolor{blond}\textbf{73.0} & \cellcolor{blond}\textbf{37.7} & \cellcolor{blond}\textbf{59.3} & \cellcolor{blond}\textbf{95.5} & \cellcolor{blond}\textbf{81.3} & \cellcolor{blond}\textbf{29.1} & \cellcolor{blond}\textbf{67.2} \\
& text-only (S) & 73.1 & \textbf{51.4} & \textbf{88.5} & 57.4 & \textbf{93.5} & \textbf{48.3} & 93.4 & 95.6 & 87.9 & 73.5 & 40.2 & 59.7 & 95.4 & 77.5 & 28.7 & 70.9 \\
% \rowcolor{blond}
& \cellcolor{blond}Ours (S,D)& \cellcolor{blond}\textbf{76.0} & \cellcolor{blond}50.8 & \cellcolor{blond}85.5 & \cellcolor{blond}\textbf{59.8} & \cellcolor{blond}92.2 & \cellcolor{blond}45.3 & \cellcolor{blond}\textbf{94.0} & \cellcolor{blond}\textbf{96.4} & \cellcolor{blond}\textbf{89.1} & \cellcolor{blond}\textbf{77.5} & \cellcolor{blond}\textbf{42.7} & \cellcolor{blond}\textbf{63.1} & \cellcolor{blond}\textbf{96.3} & \cellcolor{blond}\textbf{84.7} & \cellcolor{blond}\textbf{31.2} & \cellcolor{blond}\textbf{72.3} \\
\bottomrule



% \label{tab:vague}
\end{tabular}
\setlength{\tabcolsep}{1.4pt}
}
